Subword Regularization: An Analysis of Scalability and Generalization for End-to-End Automatic Speech Recognition

Subwords are the most widely used output units in end-to-end speech recognition. They combine the best of two worlds by modeling the majority of frequent words directly and at the same time allow open vocabulary speech recognition by backing off to shorter units or characters to construct words unseen during training. However, mapping text to subwords is ambiguous and often multiple segmentation variants are possible. Yet, many systems are trained using only the most likely segmentation. Recent research suggests that sampling subword segmentations during training acts as a regularizer for neural machine translation and speech recognition models, leading to performance improvements. In this work, we conduct a principled investigation on the regularizing effect of the subword segmentation sampling method for a streaming end-to-end speech recognition task. In particular, we evaluate the subword regularization contribution depending on the size of the training dataset. Our results suggest that subword regularization provides a consistent improvement of (2-8%) relative word-error-rate reduction, even in a large-scale setting with datasets up to a size of 20k hours. Further, we analyze the effect of subword regularization on recognition of unseen words and its implications on beam diversity.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> alpha_nbest_chance.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color1}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color2}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}
\definecolor{color3}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}

\begin{axis}[
axis line style={white!80!black},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
x grid style={white!80!black},
xlabel={alpha},
xmajorgrids,
xmajorticks=false,
xmin=0.04625, xmax=1.22875,
xtick style={color=white!15!black},
y grid style={white!80!black},
ylabel={chance},
ymajorgrids,
ymajorticks=false,
ymin=-0.035159800975, ymax=0.906930303475,
ytick style={color=white!15!black}
]
\path [draw=white!50.1960784313725!black, line width=0.48pt, dash pattern=on 4.44pt off 1.92pt]
(axis cs:0.25,-0.235159800975)
--(axis cs:0.25,0.2681599259);

\path [draw=white!50.1960784313725!black, line width=0.48pt, dash pattern=on 4.44pt off 1.92pt]
(axis cs:-0.15375,0.2681599259)
--(axis cs:0.25,0.2681599259);

\addplot [line width=0.48pt, color0, forget plot]
table {%
0.1 0.454225719
0.125 0.3891093731
0.15 0.3313426077
0.175 0.2803530395
0.2 0.2390585691
0.225 0.2033270895
0.25 0.1727600992
0.275 0.1482562125
0.3 0.1277935207
0.325 0.1112409756
0.35 0.0968093053
0.375 0.0860684663
0.4 0.0756031051
0.425 0.0676223561
0.45 0.0613158606
0.475 0.0544798076
0.5 0.050141748
0.525 0.045341
0.55 0.0422546118
0.575 0.0390585735
0.6 0.0354987979
0.625 0.0327146314
0.65 0.0306231622
0.675 0.0285209958
0.7 0.0265980214
0.725 0.0255308915
0.75 0.023752341
0.775 0.0227039307
0.8 0.0215726122
0.825 0.0194704458
0.85 0.0178710893
0.875 0.0171302482
0.9 0.0162423104
0.925 0.0157341529
0.95 0.0149692427
0.975 0.0141695645
1 0.0133939553
1.025 0.0130649908
1.05 0.0124418298
1.075 0.0113559775
1.1 0.0105750198
1.125 0.0099545335
1.15 0.0095212627
1.175 0.007764108
};
\addplot [line width=0.48pt, color1, forget plot]
table {%
0.1 0.6851270199
0.125 0.5866488218
0.15 0.4925193787
0.175 0.4153035581
0.2 0.3431345224
0.225 0.2856057882
0.25 0.2361219525
0.275 0.1964295208
0.3 0.1666167378
0.325 0.142102167
0.35 0.1204172224
0.375 0.1047793552
0.4 0.0901872143
0.425 0.0791655555
0.45 0.0706445575
0.475 0.061695639
0.5 0.0547017902
0.525 0.0495480075
0.55 0.044428993
0.575 0.0414656326
0.6 0.0369029157
0.625 0.0348167941
0.65 0.0322144963
0.675 0.0308986362
0.7 0.0280984212
0.725 0.0263599884
0.75 0.0246376041
0.775 0.02292859
0.8 0.0220673978
0.825 0.0197111536
0.85 0.0188178662
0.875 0.0173870027
0.9 0.0165391825
0.925 0.0156271737
0.95 0.0156271737
0.975 0.0142096821
1 0.0138004813
1.025 0.0128617277
1.05 0.0126584647
1.075 0.0111206202
1.1 0.0107007222
1.125 0.010320941
1.15 0.0096603371
1.175 0.0080529554
};
\addplot [line width=0.48pt, color2, forget plot]
table {%
0.1 0.7781625986
0.125 0.6596924067
0.15 0.5533431172
0.175 0.4572158456
0.2 0.37610057
0.225 0.3087483346
0.25 0.2557956576
0.275 0.2110912055
0.3 0.1745707393
0.325 0.147336185
0.35 0.1251430809
0.375 0.1084701791
0.4 0.0925220624
0.425 0.0805028081
0.45 0.0697699934
0.475 0.0625916049
0.5 0.0560738184
0.525 0.0508344471
0.55 0.044814121
0.575 0.0418641344
0.6 0.0371569954
0.625 0.0347098149
0.65 0.0322760083
0.675 0.0297887139
0.7 0.028363198
0.725 0.0263920836
0.75 0.024375502
0.775 0.0232254621
0.8 0.0218534376
0.825 0.0194490515
0.85 0.0183177311
0.875 0.0175180528
0.9 0.0170660596
0.925 0.0157421771
0.95 0.0153383259
0.975 0.0145038776
1 0.0143728266
1.025 0.0131425513
1.05 0.0125033427
1.075 0.0113533027
1.1 0.0103664082
1.125 0.0103904791
1.15 0.0093875369
1.175 0.0077828295
};
\addplot [line width=0.48pt, color3, forget plot]
table {%
0.1 0.864108026
0.125 0.7312169075
0.15 0.6064108014
0.175 0.496493727
0.2 0.4054399431
0.225 0.3314709961
0.25 0.2681599259
0.275 0.2198689431
0.3 0.1814255118
0.325 0.1517090201
0.35 0.1272586286
0.375 0.1085076258
0.4 0.093685478
0.425 0.0806552544
0.45 0.0714228377
0.475 0.0627681166
0.5 0.0562583581
0.525 0.0501390733
0.55 0.0461781211
0.575 0.0415137745
0.6 0.038443435
0.625 0.0354693756
0.65 0.0322412401
0.675 0.030123027
0.7 0.0281465631
0.725 0.025573682
0.75 0.024782028
0.775 0.0240064189
0.8 0.0216127299
0.825 0.019443702
0.85 0.0181759838
0.875 0.0168948919
0.9 0.0162530094
0.925 0.0161219575
0.95 0.0147579564
0.975 0.0144289918
1 0.0139636267
1.025 0.0130810374
1.05 0.0127012571
1.075 0.0111794602
1.1 0.0104894359
1.125 0.010500134
1.15 0.0095105646
1.175 0.0076624765
};
\end{axis}

\end{tikzpicture}

